On the Generalization Capability of Temporal Graph Learning Algorithms: Theoretical Insights and a Simpler Method

Temporal Graph Learning (TGL) has become a prevalent technique across diverse real-world applications, especially in domains where data can be represented as a graph and evolves over time. Although TGL has recently seen notable progress in algorithmic solutions, its theoretical foundations remain largely unexplored. This paper aims at bridging this gap by investigating the generalization ability of different TGL algorithms (e.g., GNN-based, RNN-based, and memory-based methods) under the finite-wide over-parameterized regime. We establish the connection between the generalization error of TGL algorithms and "the number of layers/steps" in the GNN-/RNN-based TGL methods and "the feature-label alignment (FLA) score", where FLA can be used as a proxy for the expressive power and explains the performance of memory-based methods. Guided by our theoretical analysis, we propose Simplified-Temporal-Graph-Network, which enjoys a small generalization error, improved overall performance, and lower model complexity. Extensive experiments on real-world datasets demonstrate the effectiveness of our method. Our theoretical findings and proposed algorithm offer essential insights into TGL from a theoretical standpoint, laying the groundwork for the designing practical TGL algorithms in future studies.

==> section/subfiles/gnn_setup.tex <==
Let us define the node features as $\mathbf{x}_i\in\mathbb{R}^d$, the weight matrices as $\mathbf{W}^{(1)} \in \mathbb{R}^{m \times d}$, $\mathbf{W}^{(\ell)} \in \mathbb{R}^{m\times m}, \forall \ell\in\{2,\ldots, L-1\}$, and $\mathbf{W}^{(L)} \in \mathbb{R}^{1\times m}$, and
$\alpha \in \{0, 1\}$ is a binary variable controls whether using residual connection or not. 
We denote prediction of node $i$ as $f_i(\bm{\theta}) = \mathbf{h}_i^{(L)}$ and $\bm{\theta} = \{\mathbf{W}^{(\ell)}\}_{\ell=1}^{L}$, which is recursively computed by
\begin{equation*} \label{eq:main_forward}
    \mathbf{h}_i^{(\ell)} = \begin{cases}
    \sigma(\mathbf{W}^{(1)} \sum_{j\in\mathcal{N}(i)} P_{ij} \mathbf{x}_j) & \text{ if } \ell = 1 \\ 
    \sigma(\mathbf{W}^{(\ell)} \sum_{j\in\mathcal{N}(i)} P_{ij} \mathbf{h}_j^{(\ell-1)}) + \alpha \mathbf{h}_i^{(\ell-1)} & \text{ if } \ell \in[ 2, L-1]\\ 
    \mathbf{W}^{(L)}\mathbf{h}_i^{(L-1)}   & \text{ if } \ell = L 
    \end{cases}
\end{equation*}
where $\sigma(\cdot)$ is the activation function (e.g., ReLU, LeakyReLU, Sigmoid, Tanh) and $P_{ij}$ is the $i$th row and $j$th column of the propagation matrix (e.g., $P_{ij}=1/|\mathcal{N}(i)|$ for row normalized propagation matrix and $P_{ij}=1/\sqrt{|\mathcal{N}(i)||\mathcal{N}(j)|}$ for symmetric normalized propagation matrix).





==> section/subfiles/memory_setup.tex <==
Let us define $h_i^t < t$ as the last timestamp of node $i$ before timestamp $t$ that node $i$ interact with other nodes.
Let us define $\mathbf{e}_{ij}^t \in \mathbb{R}^d$ as the link features $\mathbf{e}_{ij}^t$ between node $i,j$ at time $t$, which includes the timestamp information as used in~\cite{TGAT}.  
When an interaction happens between node $i$ and node $j$ at time $t$, we compute the most recent representation of node $i, j$ at time $t$ as $\mathbf{s}_i(t), \mathbf{s}_j(t)$. For example,  $\mathbf{s}_i(t) = \text{RNN}\left(\mathbf{s}_i^+(h_i^t), \mathbf{s}_j^+(h_j^t), \mathbf{e}_{ij}(t)\right)$ is computed by
\begin{equation*}
    \mathbf{s}_i(t) = \sigma\Big(\frac{\mathbf{W}^{(1)} \mathbf{s}_i^+(h_i^t)}{3} + \frac{\mathbf{W}^{(2)} \mathbf{s}_j^+(h_j^t)}{3} + \frac{\mathbf{W}^{(3)} \mathbf{e}_{ij}(t)}{3} \Big),
\end{equation*}
where $\mathbf{s}_i(0) = \mathbf{W}^{(0)} \mathbf{x}_i$ and $\mathbf{s}_i^+(h_i^t) = \text{StopGrad}(\mathbf{s}_i(t))$ as the memory block of node $i$ at timestamp $h_i^t$ and $\mathbf{W}^{(0)} \in \mathbb{R}^{m \times d}$ is a random initialized non-trainable projection matrix.
Then, we make  the final prediction by
\begin{equation*}
    f_i^t(\bm{\theta}) = \mathbf{h}_i(t) = \mathbf{W}^{(4)} \mathbf{s}_i(t),~
    \bm{\theta} = \{ \mathbf{W}^{(1)}, \ldots, \mathbf{W}^{(4)}\}
\end{equation*}
where $\mathbf{W}^{(1)}, \mathbf{W}^{(2)}\in\mathbb{R}^{m\times m}$, $\mathbf{W}^{(3)} \in \mathbb{R}^{m \times d}$ and $\mathbf{W}^{(4)} \in \mathbb{R}^m$.




==> section/subfiles/rnn_setup.tex <==
Let us suppose a sequence of events are sampled $\mathcal{S}_i(t)\{ \mathbf{v}_1, \ldots, \mathbf{v}_{L-1}\}$ of length $L-1$ at time $t$ and we assume each $\mathbf{v}_\ell$ includes the timestamp information. For example in CAW~\cite{CAW}, the  timestamp difference of two adjacent events are encoded as event features. Then, the RNN is used to recursively aggregate its information into $\mathbf{h}_{L-1}$  by 
\begin{equation*}
    \mathbf{h}_\ell = \begin{cases}
    \mathbf{0}_m & \text{~if~}\ell=0 \\
    \sigma \left( \frac{\mathbf{W}^{(1)} \mathbf{h}_{\ell-1}}{2}  +  \frac{\mathbf{W}^{(2)} \mathbf{x}_\ell}{2}  \right) + \alpha \mathbf{h}_{\ell-1} & \text{~if~}\ell \in [L-1] \\
    \end{cases} 
\end{equation*}
where $\mathbf{x}_\ell = \mathbf{W}^{(0)} \mathbf{v}_\ell,~\forall \ell\in[L-1]$.
Finally, the prediction on the sequence is computed by 
\begin{equation*}
    f_i^t(\bm{\theta}) = \mathbf{W}^{(3)} \mathbf{h}_{L-1}(t),~
    \bm{\theta} = \{\mathbf{W}^{(1)},\mathbf{W}^{(2)},\mathbf{W}^{(3)}\}
\end{equation*}
where $\mathbf{W}^{(1)}, \mathbf{W}^{(2)} \in \mathbb{R}^{m \times m}$ and $\mathbf{W}^{(3)} \in \mathbb{R}^{1\times m}$ are trainable weight parameters, and $\mathbf{W}^{(0)} \in \mathbb{R}^{m\times d}$ is fixed without training.
